Performance Evaluation and Modeling of Cryptographic Libraries for MPI Communications

In order for High-Performance Computing (HPC) applications with data security requirements to execute in the public cloud, the cloud infrastructure must ensure the privacy and integrity of data. To meet this goal, we consider incorporating encryption in the Message Passing Interface (MPI) library. We empirically evaluate four contemporary cryptographic libraries, OpenSSL, BoringSSL, Libsodium, and CryptoPP using micro-benchmarks and NAS parallel benchmarks on two different networking technologies, 10Gbps Ethernet and 40Gbps InfiniBand. We also develop accurate models that allow us to reason about the performance of encrypted MPI communication in different situations and give guidance on how to improve encrypted MPI performance.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> model_discussion.tex <==

%\subsection{Using model to predict performance}

\subsection{Discussion}


The simplicity of the model allows us to give an intuitive explanation for the performance of encrypted Ping-Pong, 
across different cryptographic libraries and different platforms. 
For reasonably large messages, 
$\Tcomm(m)$ and $\Ted(m)$ are dominated by $\bcomm \cdot m$ and $\bed \cdot m$ respectively, 
and thus the encryption overhead  (for throughput) is 
\[ 
   \frac{\Ted(m)}{\Tcomm(m)} \approx \frac{\bed \cdot m}{\bcomm \cdot m} = \frac{\bed}{\bcomm} \enspace. 
\] 
For example, the overhead of BoringSSL for large messages is predicted to be $80\%$ in Ethernet, 
and $221\%$ in Infiniband, which is consistent with the Ping-Pong benchmarks in \secref{sec:perf}. 



\smallskip
As shown above, there is currently a huge gap between what single-core encryption can provide
and what a high-speed network can consume. 
A possible way to bridge that gap
is to encrypt/decrypt via multiple threads. 
In addition, in the current implementation of encrypted Ping Pong, 
the receiver stays idle while the sender encrypts the message, and vice versa. 
If one can somehow pipeline the encryption and decryption (for example, by chopping the message into small segments as in streaming encryption~\cite{C:HRRV15})
then the overhead may be reduced even further. 
\iffalse
The performance of encrypted Ping Pong for $k$ threads then resembles that of encrypted Multiple Pair for $k$ pairs of senders and receivers, 
which we provide a model in \secref{sec:multipairs}. 
\fi


\iffalse
As shown above, there is currently a huge gap between what single-core encryption can provide
and what a high-speed network can consume. 
A possible way to bridge that gap
is to encrypt/decrypt via multiple threads. 
Ideally, if we use $k$ threads to encrypt/decrypt then we might reduce the overhead to $\bed / (k \cdot \bcomm)$. 
\iffalse
Indeed, as illustrated in the OSU Multiple-Pair benchmarks, 
using 8 threads for encryption/decryption would result in negligible overhead, even in Infiniband. 
\fi
Additionally, in the current implementation of encrypted MPI, 
the receiver stays idle while the sender encrypts the message, 
and vice versa. 
If one can somehow pipeline the encryption and decryption (for example, by chopping the message into small segments as in streaming encryption~\cite{C:HRRV15})
then the overhead may be reduced even further, reaching $\bed / (2k \cdot \bcomm)$.
\fi



\iffalse
 In particular, if we have $k$ threads for encryption/decryption, 
the overhead would be reduced to about $\frac{1}{1 + k \cdot \Red / \Rcomm}$. 

Indeed, as illustrated in the OSU Multiple-Pair benchmarks, 
for $k = 8$, the overhead is negligible. 
\fi

\iffalse
Additionally, in the current implementation of encrypted MPI, 
the receiver stays ideal while the sender encrypts the message, 
and vice versa. 
If one can somehow pipeline the encryption and decryption (for example, by chopping the message into multiple segments), the overhead will be reduced even further, 
potentially to $\frac{1}{1 + 2k \cdot \Red / \Rcomm}$.
\fi





\iffalse
\subsection{Discussion}

As demonstrated in the previous sub-sections, the Hockney model can predict the performance
of secure MPI point-to-point communication accurately; and the parameters for the Hockney
models can be derived from the models for the MPI library and encryption library
independently. Here, we will use BoringSSL to reason about the performance trend for
secure MPI communication as the technology advances using the models under the
following assumptions, which reflect the current trend of technology advancements. 

\begin{itemize}
\item Single core encryption performance will not drastically improve since the single
  core computation performance is unlikely to drastically improve in the future. 
\item Communication performance for both Ethernet and InfiniBand will continue to improve
  both in the latency and bandwidth.
\end{itemize}

\noindent
    {\bf Secure MPI communication of small messages}. Using the Hockney model, the time
    to communicate a small message is dominated by the $\alpha$ term. As shown
    in Tables~\ref{tab:naive_comm}, \ref{tab:naive_comp}, and \ref{tab:securecomm},
    the $\alpha$ value for small messages is $33.0385\mu s$ for Ethernet and $3.5045\mu s$
    for InfiniBand. Both are significantly larger
    than the $\alpha$ value for BoringSSL ($0.5474\mu s$). As the networking
    technology advances, the communication latency will continue to decrease, and the
    performance of secure MPI communication of small messages will also continue to
    improve. 

\noindent
    {\bf Secure MPI communication of large messages}. Using the Hockney model, the time
    to communicate a large message is dominated by the $\beta$ term. Values of $\beta$ in
    Tables~\ref{tab:naive_comm}, \ref{tab:naive_comp}, and \ref{tab:noleland_comm_comp}, 
    for large messages is
    $0.000903$ for 10Gbps Ethernet, $0.000327$ for 40 Gbps InfiniBand, and $0.000087$ for 100Gbps InfiniBand.
    As the technology advances, the
    bandwidth will continue to increase and the $\beta$ value will continue to
    decrease in future networks. As the same time, the $\beta$ value for BoringSSL is
    around $0.0007$ which is roughly equivalent to a bandwidth of 13Gbps and it decreases to around 0.0003 in a more recent system. This value is unlikely to improve significantly in the future. This indicates that
    for secure MPI communication of large message, the encryption will dominate the total
    time in the current and future generation systems. Furthermore, unless there is
    technology breakthrough for encryption, communication link with large bandwidth will not
    significantly improve performance of single secure MPI communication.
    *****TODO: Is it still true regarding the decrease in the beta value on Noleland (from 0.0007 to 0.0003)?

\noindent
     {\bf Impact of adding security to MPI communication}. Using the Hockney model,
     one can also estimate the overhead for adding security to MPI communication. For
     large messages, the throughput is equal to $\frac{1}{\beta}$. Table~\ref{tab:overhead}
     lists the throughput of adding security to MPI communication on the current
     10Gbps Ethernet, 40Gbps InfiniBand, and 100Gbps InfiniBand. As the
     table shows, for 10Gbps Ethernet, the encrypting and decrypting speed is roughly
     equal to the network speed, adding security incurs 44\% of overhead. As the network
     speed increases, for 100Gbps InfiniBand, the overhead percentage increases to 80\%:
     the encrypting and decrypting time dominates the total secure communication time.


\begin{table}
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
  \hline
  Network & $\beta_{comm}$ & $T_{comm}$ & $\beta_{sec}$ & $T_{sec}$ & $\beta_{comb}$ & $T_{comb}$ & Overh. \\
  \hline
  10G Eth & 0.000903 & 1.10Gbps & 0.000723 & 1.38Gbps & 0.001626 & 614Mbps & 44\%\\
  \hline
  40G IB & 0.000327 & 3.05Gbps & 0.000723 & 1.38Gbps & 0.001049 & 953Mbps & 68\% \\
  \hline
  100G IB & 0.000087 & 11.44Gbps & 0.000363 & 2.75Gbps & 0.000450 & 2.21Gbps & 80\%\\
  \hline
  \end{tabular}
\caption{Overhead of adding security to MPI communication}
\label{tab:overhead}
\end{table}

\noindent
    {\bf Effectiveness of the pipelining communication techniques}. In a library routine
    with significant computation and communication such as transferring large messages,
    pipelined communication is a mechanism that has proven to be effective
    in many situations \cite{Patarasuk:2009}. In the context of secure MPI communication,
    pipelined communication can be realized as follows. To communicate a large message,
    the message is chopped into a number of segments. The system can then encrypt,
    send/receive, and decrypt the segments in a pipeline manner. As such,
    the communication and encryption/decryption operations can be overlapped, which in
    theory allows either the communication or encryption/decryption time to be removed
    from the critical path of the secure MPI communication.

    Table~\ref{tab:pipelined}
    shows the potential impact of pipelined communication when it is applied to secure
    MPI communication on different networks under the idealistic
    assumption that pipelining does not
    introduce additional overheads. For 10Gbps Ethernet, this technique can be very
    effective, completely removing the encryption and decryption overhead from the secure
    MPI communication since the encryption and decryption operations can be overlapped with
    the communication operation. For the faster 40Gbps or 100Gbps InfiniBand, however,
    pipelined communication will not be effective because the encryption and decryption
    dominate the total secure communication time. For example, for 100Gbps InfiniBand,
    pipelined communication only reduces the overhead for adding security to MPI
    communication from 80\% to 75\%. 
    
    To demonstrate the effectiveness of this pipelining technique, we measured the latency
    of pipelined secure MPI point-to-point communication when chopping large messages to 64KB chunks.
    Figure~\ref{fig:pipelining} compares the effect of this technique by comparing the throughput in this scenario with the throughput when we don't use pipelining. The throughputs for unencrypted and secure MPI point-to-point communication on 10Gbps Ethernet and 40Gbps Infiniband networks were presented in Figure~\ref{fig:pingpong_ethernet}. We use the BoringSSL library with 256-bit keys for all the encryption/decryptions for these experiments. Figure~\ref{fig:pipelining} shows that pipelining communication is much more effective on 10Gbps Ethernet for reducing the performance gap 
    between unencrypted and secure MPI point-to-point communication.
    
    
\begin{figure}
\centering
 \subfloat[10Gbps Ethernet]{
        \includegraphics[width=0.50\textwidth]{Naive_Model_Figures/e_pipelined.eps}
    }
    \subfloat[40Gbps Infiniband]{
        \includegraphics[width=0.50\textwidth]{Naive_Model_Figures/i_pipelined.eps}
    }
    \caption{Effect of using pipelining communication techniques on 10Gbps Ethernet and 40Gbps Infiniband networks}
   
\label{fig:pipelining}
\end{figure}

    
    

\begin{table}
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
  \hline
  Network & $\beta_{comm}$ & $T_{comm}$ & $\beta_{sec}$ & $T_{sec}^{p}$ & $\beta_{comb}^{p}$ & $T_{comb}$ & Overh. \\
  \hline
  10G Eth & 0.000903 & 1.1Gbps & 0.000723 & 1.38Gbps & 0.000903 & 1.1Gbps & 0\%\\
  \hline
  40G IB & 0.000327 & 3.05Gbps & 0.000723 & 1.38Gbps & 0.000723 & 1.38GBps & 54\% \\
  \hline
  100G IB & 0.000087 & 11.44Gbps & 0.000363 & 2.75Gbps & 0.000363 & 2.75GBps & 75\%\\
  \hline
  \end{tabular}
\caption{Effective of pipelined communication}
\label{tab:pipelined}
\end{table}

\noindent
    {\bf A technique for improving secure MPI communication on high-speed networks}.
    Given that a single thread encryption and decryption performance is unlike
    to improve in the future, the only effective scheme to improve the
    performance of secure MPI communication on high-speed networks,
    such as 100Gbps network, is to improve the encryption/decryption throughput. 
    Using multiple threads to simultaneously
    encrypting and decrypting a large message will achieve this effect.
    As technology advances,
    the future CPU will likely to have many more cores, some may not
    be used to run MPI tasks and can be used to help the communication.
    This technique explores such an opportunity. 

    Let us assume the message size is $m$ bytes and there are $N$ additional
    cores that can be used to help communication. The message is
    partitioned into $N+1$ segments; and each core will be working on the
    encryption and decryption of the $N+1$ segments, potential improve the
    encryption and decryption throughput by a factor of $N+1$. 

    Table~\ref{tab:multi}
    shows the potential impact of multi-threaded secure MPI
    communication when it is applied to 100Gbps InfiniBand networks.
    With 8 cores, the overhead to security is reduced to 50\%. In this
    situation, when the communication is overlapped with encryption and decryption,
    the performance can in theory be at the same speed as the raw network speed. 

\begin{table}
\centering
\begin{tabular}{|l|l|l|l|}
  \hline
  Extra-core & $\beta_{comb}^{p}$ & $T_{comb}$ & Overhead \\
  \hline
  0 & 0.0008 & 1.25Gbps & 88\%\\
  \hline
  1 & 0.00045 & 2.22Gbps & 78\%\\
  \hline
  3 & 0.00033 & 3Gbps    & 70\%\\
  \hline
  7 & 0.0002  & 5Gbps    & 50\%\\
  \hline
  \end{tabular}
\caption{Effective of multi-threaded encryption and decryption on 100Gbps InfiniBand}
\label{tab:multi}
\end{table}

\fi

